The Stronger the Diffusion Model, the Easier the Backdoor: Data Poisoning to Induce Copyright Breaches Without Adjusting Finetuning Pipeline

The commercialization of text-to-image diffusion models (DMs) brings forth potential copyright concerns. Despite numerous attempts to protect DMs from copyright issues, the vulnerabilities of these solutions are underexplored. In this study, we formalized the Copyright Infringement Attack on generative AI models and proposed a backdoor attack method, SilentBadDiffusion, to induce copyright infringement without requiring access to or control over training processes. Our method strategically embeds connections between pieces of copyrighted information and text references in poisoning data while carefully dispersing that information, making the poisoning data inconspicuous when integrated into a clean dataset. Our experiments show the stealth and efficacy of the poisoning data. When given specific text prompts, DMs trained with a poisoning ratio of 0.20% can produce copyrighted images. Additionally, the results reveal that the more sophisticated the DMs are, the easier the success of the attack becomes. These findings underline potential pitfalls in the prevailing copyright protection strategies and underscore the necessity for increased scrutiny to prevent the misuse of DMs.

==> tables/SD_variants.tex <==
\begin{table}[h]
\centering
\scalebox{0.8}{
\begin{tabular}{l|ccccc}
\toprule
& {SD V1.1} & {SD V1.2} & {SD V1.3} & {SD V1.4} & {SD V1.5} \\ \hline
Caterpie                          & 954                         & 684                         & 315                         & 288                         & 288      
\\
Bulbasaur & 525                         & 540                         & 420                         & 435                         & 360                         \\ 
\bottomrule
\end{tabular}
}
\caption{Number of steps required by various Stable Diffusion versions to achieve a successful attack for the first time (SSCD Similarity $> 0.5$).}
\label{tab:dm_variant}
\end{table}


==> tables/effectivenss_tab.tex <==
\begin{table*}[h]
\centering
\setlength{\tabcolsep}{5pt}{
\scalebox{0.8}{
\begin{tabular}{l|c|c|c|c|c|c}
\toprule
% & w/o FT                    & on Train set              & Bul. Poisoning            & \begin{tabular}[c]{@{}l@{}}Bul. Poisoning\\ w. Guidance Set\end{tabular} & Cate. Poisoning           & \begin{tabular}[c]{@{}l@{}}Cate. Poisoning\\ w. Guidance Set\end{tabular} \\ \hline
% {Bulbasaur Prompt} & {24.55} &{30.85} & {39.17} & \textbf{51.58}                                          & {16.92} & {20.61}                                           \\ 
% \hline
% {Caterpie Prompt}  & {15.48} & {28.15} & {14.97} & {17.47}                                          & {25.64} & \textbf{59.37}                                           \\ 
& w/o FT                    & On training data    & \begin{tabular}[c]{@{}l@{}}Bul. poisoning\\data \end{tabular}          & \begin{tabular}[c]{@{}l@{}}Bul. poisoning\\ + auxiliary data\end{tabular} & \begin{tabular}[c]{@{}l@{}}Cate. poisoning\\data \end{tabular}          & \begin{tabular}[c]{@{}l@{}}Cate. poisoning\\ + auxiliary data\end{tabular} \\ \hline
{Caterpie prompt}  & {0.155} & {0.282} & {0.150} & {0.175} & {0.256} & \textbf{0.594}  \\ 
{Bulbasaur prompt} & {0.246} &{0.309} & {0.392} & \textbf{0.516} & {0.169} & {0.206}  \\ 
\bottomrule                 
\end{tabular}
}
}
\caption{SSCD similarity between target images and those generated by the SD fine-tuned across various datasets. Beginning from the fourth column (poisoned dataset), the clean training set is used.}
\label{tab:attack_effect}
\end{table*}


==> tables/stealthy_poison.tex <==
\begin{table*}[h]
\centering
% \scalebox{0.8}{
\setlength{\tabcolsep}{4pt}{
\begin{tabular}{ccccccc}
\toprule
\multicolumn{1}{l|}{}                          &             & \multicolumn{1}{l}{Train-Avg.} & Train-Max. & Poison-Avg. & Poison-Max. & Rank of Poison-Max. in Train \\
% \cline{1-5} 
\toprule
\multicolumn{1}{c|}{\multirow{3}{*}{\rotatebox{90}{Caterpie}}}    & SSCD & 0.223 & 0.442 & 0.158 &  0.367  &  26        \\
\multicolumn{1}{c|}{}                         & CLIP &  0.731  & 0.884 & 0.628 &  0.803  &  81    \\
\multicolumn{1}{c|}{}                         & DINO &  0.614  &0.804 & 0.526 &  0.716  & 64       \\
\midrule
\multicolumn{1}{c|}{\multirow{3}{*}{\rotatebox{90}{Bulbas.}}}    & SSCD & 0.291 & 0.492 & 0.264 & 0.431 &   35        \\
\multicolumn{1}{c|}{}                         & CLIP &  0.739  & 0.911 & 0.669 &  0.837  &  57    \\
\multicolumn{1}{c|}{}                         & DINO &  0.555  & 0.779 & 0.511  &  0.641  & 79    \\
\bottomrule
\end{tabular}
}
% }
\vspace{3pt}
\caption{The SSCD Similarity between target images and images within different datasets and the rank of most similar poisoning image in the training set.}
\label{tab:poisoning_data_stat}
\end{table*}
